VideoMemBench: How Well Do MLLMs Remember in Video Conversations?

Multimodal large language models (MLLMs) can now process hour-long videos, making extended multi-turn dialogue over a single video a natural mode of use. Sustaining such a dialogue requires more than answering each question in isolation: the model must retrieve and reuse information established earlier in the conversation, both what it has seen and what it has said, an ability we term in-context video memory. Existing video QA benchmarks leave this ability unmeasured: their questions are mutually independent, never reference one another, and each is answerable from the video alone, so nothing ever requires carrying information across turns. We introduce VideoMemBench, in which each sample pairs a single video with a long multi-turn dialogue, whose turns are connected by typed cross-turn dependencies: an Episodic Dependency refers back to a visual episode described in an earlier turn, probing memory of what the model has seen, while an Answer Dependency builds on the model's own earlier answer, probing memory of what the model has said. Every dependency is verified considering two properties: 1) necessity, meaning the question cannot be answered without its earlier turns, and 2) non-leakage, meaning the question does not restate the information from its earlier turns. To enforce these properties, we design a construction pipeline with three LLM roles: a planner, a generator, and a judger, with each dialogue reviewed by human experts. VideoMemBench comprises 326 videos with 2,476 turns, of which 1,387 depend on earlier turns, including multi-parent dependencies and long-range call-back. Among over 20 evaluated open- and closed-source MLLMs, Claude Opus 5 performs the best with an overall score of only 45.7%, highlighting the challenge of in-context video memory. Our dataset and evaluation are released.

==> authors.tex <==
\makeatletter
\iflatexml
\author{%
\begin{minipage}[t]{\linewidth}
\raggedright
Zhengdong Hu\textsuperscript{1,*}, Chao Wang\textsuperscript{1,*},
Kaituo Feng\textsuperscript{2}, Huanjin Yao\textsuperscript{3},
Mingfei Lu\textsuperscript{1}, Hehe Fan\textsuperscript{4},
Yi Yang\textsuperscript{4,\dagger}\\[5pt]
\textsuperscript{1}University of Technology Sydney, Sydney, Australia\\
\textsuperscript{2}The Chinese University of Hong Kong, Hong Kong, China\\
\textsuperscript{3}The Hong Kong University of Science and Technology, Hong Kong, China\\
\textsuperscript{4}Zhejiang University, Hangzhou, China\\[5pt]
\textsuperscript{*}Equal contribution.\\
\textsuperscript{\dagger}Corresponding author.
\end{minipage}%
}
\else
\author{%
\begin{minipage}[t]{\linewidth}
\raggedright
\renewcommand{\@makefnmark}{\hbox{\@textsuperscript{\normalfont\@thefnmark}}}%
Zhengdong Hu$^{1,}$\thanks{Equal contribution.}, Chao Wang$^{1,}$\footnotemark[1], Kaituo Feng$^{2}$, Huanjin Yao$^{3}$,
Mingfei Lu$^{1}$, Hehe Fan$^{4}$, Yi Yang$^{4,}$\thanks{Corresponding author.}\\[5pt]
\normalfont\small
$^{1}$\,University of Technology Sydney, Sydney, Australia\\
$^{2}$\,The Chinese University of Hong Kong, Hong Kong, China\\
$^{3}$\,The Hong Kong University of Science and Technology, Hong Kong, China\\
$^{4}$\,Zhejiang University, Hangzhou, China
\end{minipage}%
}
\fi
\makeatother
\hypersetup{pdfauthor={Zhengdong Hu, Chao Wang, Kaituo Feng, Huanjin Yao, Mingfei Lu, Hehe Fan, Yi Yang}}

